DP-SGD with weight clipping

Recently, due to the popularity of deep neural networks and other methods whose training typically relies on the optimization of an objective function, and due to concerns for data privacy, there is a lot of interest in differentially private gradient descent methods. To achieve differential privacy guarantees with a minimum amount of noise, it is important to be able to bound precisely the sensitivity of the information which the participants will observe. In this study, we present a novel approach that mitigates the bias arising from traditional gradient clipping. By leveraging a public upper bound of the Lipschitz value of the current model and its current location within the search domain, we can achieve refined noise level adjustments. We present a new algorithm with improved differential privacy guarantees and a systematic empirical evaluation, showing that our new approach outperforms existing approaches also in practice.

==> subfiles/algos/layer_sensitivity.tex <==
\begin{algorithm}[ht]
   \caption{$\textsc{LayerSensitivity}(f, \theta, u^{(\theta)})$}
   % \label{alg:\gradDpSgd-logloss-l1}
   \label{alg:layer_sensitivity}
\begin{algorithmic}[1]
  \State {\bfseries Input:} $K$ layer feed-forward model $f$, parameters $\theta$, parameter norm $u^{(\theta)}$, max input norm $X_1$, upper bound of loss Lipschitz value $l_{K+1}$.
   \For{$k=1$ {\bfseries to} $K$} \Comment{Forward pass}
   \If{$\theta_k=\emptyset$}
   \If{$k$-th layer is a normalization layer}
   \State $X_{k+1} \leftarrow \min(|x_{k+1}|^{\frac{1}{2}}, \frac{X_k}{\alpha})$ %\Comment{$\sigma^{(k+1:\grpidx)} = 1$}
   \Else\Comment{e.g., activation layer}
   \State $X_{k+1} \leftarrow X_{k}L_{x_k}$
   \EndIf
   \Else
   \State $X_{k+1} \leftarrow X_{k}u_k^{(\theta)}$
   \EndIf
   \EndFor
   \For{$k=K$ {\bfseries to} $1$} \Comment{Backward pass}
   \State $l_k\text{ }\leftarrow  l_{k+1} L_{x_k}$
   \State $\Delta_k \leftarrow l_{k+1} L_{\theta_k}$ %\Comment{$L_{\theta_k}=0$ when $\theta_k=\emptyset$}
   \EndFor
   \State {\bfseries Output:} $(\Delta_1, \dots, \Delta_{K-1}, \Delta_K)$.
\end{algorithmic}
\end{algorithm}


==> subfiles/checklist.tex <==
\section*{Checklist}

 \begin{enumerate}


 \item For all models and algorithms presented, check if you include:
 \begin{enumerate}
   \item A clear description of the mathematical setting, assumptions, algorithm, and/or model. [Yes]
   \item An analysis of the properties and complexity (time, space, sample size) of any algorithm. [Yes]
   \item (Optional) Anonymized source code, with specification of all dependencies, including external libraries. [Yes]
 \end{enumerate}


 \item For any theoretical claim, check if you include:
 \begin{enumerate}
   \item Statements of the full set of assumptions of all theoretical results. [Yes]
   \item Complete proofs of all theoretical results. [Yes]
   \item Clear explanations of any assumptions. [Yes]
 \end{enumerate}


 \item For all figures and tables that present empirical results, check if you include:
 \begin{enumerate}
   \item The code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL). [Yes]
   \item All the training details (e.g., data splits, hyperparameters, how they were chosen). [Yes]
         \item A clear definition of the specific measure or statistics and error bars (e.g., with respect to the random seed after running experiments multiple times). [Yes]
         \item A description of the computing infrastructure used. (e.g., type of GPUs, internal cluster, or cloud provider). [Yes]
 \end{enumerate}

 \item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets, check if you include:
 \begin{enumerate}
   \item Citations of the creator If your work uses existing assets. [Yes]
   \item The license information of the assets, if applicable. [Yes]
   \item New assets either in the supplemental material or as a URL, if applicable. [Not Applicable]
   \item Information about consent from data providers/curators. [Not Applicable]
   \item Discussion of sensible content if applicable, e.g., personally identifiable information or offensive content. [Not Applicable]
 \end{enumerate}

 \item If you used crowdsourcing or conducted research with human subjects, check if you include:
 \begin{enumerate}
   \item The full text of instructions given to participants and screenshots. [Not Applicable]
   \item Descriptions of potential participant risks, with links to Institutional Review Board (IRB) approvals if applicable. [Not Applicable]
   \item The estimated hourly wage paid to participants and the total amount spent on participant compensation. [Not Applicable]
 \end{enumerate}

 \end{enumerate}

